Dataset Enhancement with Instance-Level Augmentations

We present a method for expanding a dataset by incorporating knowledge from the wide distribution of pre-trained latent diffusion models. Data augmentations typically incorporate inductive biases about the image formation process into the training (e.g. translation, scaling, colour changes, etc.). Here, we go beyond simple pixel transformations and introduce the concept of instance-level data augmentation by repainting parts of the image at the level of object instances. The method combines a conditional diffusion model with depth and edge maps control conditioning to seamlessly repaint individual objects inside the scene, being applicable to any segmentation or detection dataset. Used as a data augmentation method, it improves the performance and generalization of the state-of-the-art salient object detection, semantic segmentation and object detection models. By redrawing all privacy-sensitive instances (people, license plates, etc.), the method is also applicable for data anonymization. We also release fully synthetic and anonymized expansions for popular datasets: COCO, Pascal VOC and DUTS.

==> sections/limitations.tex <==
\section{Limitations and Bias}

==> tables/coco_20.tex <==
\begin{table*}[t]
\footnotesize
\centering
\resizebox{\linewidth}{!}{\begin{tabular}{r|c|c|ccc|ccc|ccc|}
\noalign{\smallskip}
& & & \multicolumn{3}{c}{COCO \cite{mscoco}} & \multicolumn{3}{c}{Pascal VOC \cite{voc}} & \multicolumn{3}{c}{Open Images \cite{openimages}}\\
Model & Data \% & Ours & AP & AP$_{50}$ & AP$_{75}$ & AP & AP$_{50}$ & AP$_{75}$ & AP & AP$_{50}$ & AP$_{75}$\\
\hline
RT-DETR-X\cite{rtdetr} & 10 & \xmark & 0.288 & 0.428 & 0.306 & 0.445 & 0.615 & 0.478 & 0.205 & 0.255 & 0.216 \\
RT-DETR-X\cite{rtdetr} & 10 & \cmark & \textbf{0.302} & \textbf{0.443} & \textbf{0.322} & \textbf{0.467} & \textbf{0.639} & \textbf{0.499} & \textbf{0.209} & \textbf{0.258} & \textbf{0.220} \\
\hline
RT-DETR-X\cite{rtdetr} & 20 & \xmark & 0.365 & 0.524 & 0.392 & 0.536 & 0.712 & 0.575 & 0.256 & 0.309 & 0.270 \\
RT-DETR-X\cite{rtdetr} & 20 & \cmark & \textbf{0.377} & \textbf{0.540} & \textbf{0.401} & \textbf{0.560} & \textbf{0.739} & \textbf{0.601} & \textbf{0.261} & \textbf{0.313} & \textbf{0.272} \\
\hline
RT-DETR-X\cite{rtdetr} & 100 & \xmark & \textbf{0.489} & 0.667 & \textbf{0.529} & 0.671 & 0.838 & 0.719 & \textbf{0.337} & 0.386 & \textbf{0.350} \\
RT-DETR-X\cite{rtdetr} & 100 & \cmark & \textbf{0.489} & \textbf{0.668} & 0.528 & \textbf{0.674} & \textbf{0.840} & \textbf{0.724} & \textbf{0.337} & \textbf{0.387} & \textbf{0.350} \\
\noalign{\smallskip}
\end{tabular}}
\caption{ \textbf{Detector Generalization:} For a limited amount of available training data, Instance Level Augmentations improve the model generalization and performance by a large margin on all benchmarks.}
\label{t:coco_20}
\end{table*}

==> tables/rebuttal_detr.tex <==
\begin{table}[h!]
\footnotesize
\setlength{\tabcolsep}{1.5pt}
\centering
\begin{tabular}{lcccc}
\toprule
 Model & Ours & AP & AP$_{50}$ & AP$_{75}$\\
\midrule
 Deformable-DETR (single scale) & \xmark & 34.1 & 54.8 & 36.0\\
 Deformable-DETR (single scale) & \cmark & \textbf{36.2} & \textbf{55.9} & \textbf{39.0}\\
\bottomrule
\end{tabular}\vspace{-1em}
\caption{MS-COCO Object Detection results.}\label{t:rebuttal_detr}
\end{table}

==> tables/rebuttal_voc.tex <==
\begin{table}[h!]
\footnotesize
\vspace{-2em}
\setlength{\tabcolsep}{1.5pt}
\centering
\begin{tabular}{lcccccccc}
\toprule
Dataset & mIoU & airplane & bird & boat & car & person & cat & sofa\\
\midrule
 Real & 77.3 & 87.5 & 94.4 & 70.6 & 87.7 & 89.2 & 92.2 & 53.6\\
 \midrule
 Diffumask  & 57.4 & 80.7 & 86.7 & 56.9 & 74.2 & 71.0 & 79.3 & 27.8\\
 Ours  & \textbf{71.8} & \textbf{87.1} & \textbf{91.6} & \textbf{69.1} & \textbf{79.2} & \textbf{88.7} & \textbf{89.6} & \textbf{44.5}\\
\bottomrule
\label{t:rebuttal_voc}
\end{tabular}\vspace{-2em}
\caption{PASCAL VOC Semantic Segmentation results.}\label{t:rebuttal_voc}\vspace{-1.1em}
\end{table}

==> tables/rebuttal_voc_swin.tex <==
%\begin{minipage}[b]{\linewidth}\centering
\begin{table}[thb]
\tiny
\footnotesize
\centering
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{1.2}
\resizebox{\linewidth}{!}{\begin{tabular}{cc|ccccccccccccc|c}
\textbf{Real} &\textbf{Syn.} & \faPlane & \faBird & \faShip & \faBus & \faCar & \faCat &	\faChair & \faCow & \faDog & \faHorse & \faWalking & \faSheep & \faCouch & \textbf{mIoU} \\
\toprule
%\xmark & Ours & 93.6 & 89.6 & 76.0 & 92.4 & 88.1 & 94.6 & 52.9 & 90.8 & 91.9 & 92.2 & 87.2 & 93.3 & 50.6 & 80.1 \\
VOC & Diffumask & 95.6 & \textbf{94.4} & 72.3 & \textbf{96.9} & 92.9 & 96.6 & 51.5 & \textbf{96.7} & \textbf{95.5} & \textbf{96.1} & 91.5 & \textbf{96.4} & 70.2 & 84.9 \\
VOC & Ours & \textbf{95.7} & 93.9 & \textbf{76.7} & 96.8 & \textbf{93.6} & \textbf{97.5} & \textbf{57.0} & 96.1 & 95.2 & 95.1 & \textbf{91.6} & 95.8 & \textbf{71.3} & \textbf{86.2} \\
\bottomrule
\noalign{\smallskip}
\end{tabular}}%\label{t:voc_swin}
\vspace{-0.5em}
\end{table}
%\end{minipage}
